Data-Driven Inference of Representation Invariants

A representation invariant is a property that holds of all values of abstract type produced by a module. Representation invariants play important roles in software engineering and program verification. In this paper, we develop a counterexample-driven algorithm for inferring a representation invariant that is sufficient to imply a desired specification for a module. The key novelty is a type-directed notion of visible inductiveness, which ensures that the algorithm makes progress toward its goal as it alternates between weakening and strengthening candidate invariants. The algorithm is parameterized by an example-based synthesis engine and a verifier, and we prove that it is sound and complete for first-order modules over finite types, assuming that the synthesizer and verifier are as well. We implement these ideas in a tool called Hanoi, which synthesizes representation invariants for recursive data types. Hanoi not only handles invariants for first-order code, but higher-order code as well. In its back end, Hanoi uses an enumerative synthesizer called Myth and an enumerative testing tool as a verifier. Because Hanoi uses testing for verification, it is not sound, though our empirical evaluation shows that it is successful on the benchmarks we investigated.

==> listeset-module.tex <==
\begin{figure}[!t]\small%
\begin{boxed-listing}[left=-22pt]{}
module ListESet : ESET = struct
  include ListSet#\vspace*{-0.75em}#

  let rec union l = function
    | [] -> l
    | hd :: tl -> union (insert hd l) tl#\vspace*{-0.625em}#

  let rec inter l = function
    | [] -> []
    | hd :: tl -> if (lookup l hd)
                  then (hd :: (inter l tl))
                  else (inter l tl)
end
\end{boxed-listing}
\caption{A module that implements \texttt{ESET} using lists.}%
\label{fig:listset-ext-module}
\end{figure}
